3D-SSGAN: Lifting 2D Semantics for 3D-Aware Compositional Portrait Synthesis

Existing 3D-aware portrait synthesis methods can generate impressive high-quality images while preserving strong 3D consistency. However, most of them cannot support the fine-grained part-level control over synthesized images. Conversely, some GAN-based 2D portrait synthesis methods can achieve clear disentanglement of facial regions, but they cannot preserve view consistency due to a lack of 3D modeling abilities. To address these issues, we propose 3D-SSGAN, a novel framework for 3D-aware compositional portrait image synthesis. First, a simple yet effective depth-guided 2D-to-3D lifting module maps the generated 2D part features and semantics to 3D. Then, a volume renderer with a novel 3D-aware semantic mask renderer is utilized to produce the composed face features and corresponding masks. The whole framework is trained end-to-end by discriminating between real and synthesized 2D images and their semantic masks. Quantitative and qualitative evaluations demonstrate the superiority of 3D-SSGAN in controllable part-level synthesis while preserving 3D view consistency.

==> paper/inplementationdetails.tex <==
\section{Implementation Details}

In our occlusion-aware mask module, we do not use nerf weights to generate semantic segmentation mask in the first 2000 iterations, the implementation can refer Sec. \ref{ablation}. The pose $p$ used in volume rendering is sampled from Gaussian distribution, the standard deviations are 0.3 and 0.155 for yaw and pitch respectively, and the mean is $\pi/2$. In volume rendering, we need to sample several points to compose the final feature for each pixel, the number of sampled points for each pixel is 12 in training, and 36 sampled points are used in testing to achieve better view consistency and quality. The "ToDepth" layer used in local generator is a FC layer with a bias of size $64\times 64$, the bias is like a face template, which is general for all faces. Different from "ToDepth" layer, the "ToDensity" layer and "ToFeat" layer keep the setting of SemanticStyleGAN \cite{shi2022semanticstylegan}, whose size of bias is 1, to ensure the diversity of synthesis images. $\lambda_{depth}$ is set to 0.1 to control the weight of depth smoothness. 

==> paper/our_commands.tex <==

\definecolor{green}{rgb}{0, 0.5, 0}
\definecolor{orange}{rgb}{0.8, 0.6, 0.2}
\definecolor{red}{rgb}{1.0, 0.0, 0.0}
\definecolor{teal}{rgb}{0.0, 0.4, 0.4}
\definecolor{purple}{rgb}{0.65,0,0.65}
\definecolor{saffron}{rgb}{0.95,0.75,0.2}
\definecolor{turquoise}{rgb}{0.0,0.5,0.5}
\definecolor{black}{rgb}{0.0, 0.0, 0.0}
\definecolor{gray}{rgb}{0.5, 0.5, 0.5}

\newcommand{\rui}[1]{{\color{purple}#1}}
\newcommand{\wy}[1]{{\color{orange}#1}}

\newcommand{\TODO}[1]{{\color{red}#1}}

